TorchDriveEnv: A Reinforcement Learning Benchmark for Autonomous Driving with Reactive, Realistic, and Diverse Non-Playable Characters

The training, testing, and deployment, of autonomous vehicles requires realistic and efficient simulators. Moreover, because of the high variability between different problems presented in different autonomous systems, these simulators need to be easy to use, and easy to modify. To address these problems we introduce TorchDriveSim and its benchmark extension TorchDriveEnv. TorchDriveEnv is a lightweight reinforcement learning benchmark programmed entirely in Python, which can be modified to test a number of different factors in learned vehicle behavior, including the effect of varying kinematic models, agent types, and traffic control patterns. Most importantly unlike many replay based simulation approaches, TorchDriveEnv is fully integrated with a state of the art behavioral simulation API. This allows users to train and evaluate driving models alongside data driven Non-Playable Characters (NPC) whose initializations and driving behavior are reactive, realistic, and diverse. We illustrate the efficiency and simplicity of TorchDriveEnv by evaluating common reinforcement learning baselines in both training and validation environments. Our experiments show that TorchDriveEnv is easy to use, but difficult to solve.

==> figures/multi_agent.tex <==
\begin{figure*}[h!]
    \centering 
    \begin{subfigure}[b]{.48\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{assets/multi-agent-eval.pdf}  
         \caption{ }
         \label{fig:multi-agent:train}
     \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{assets/multi-agent-eval.pdf}  
         \caption{ }
         \label{fig:multi-agent:val}
     \end{subfigure}
    \caption{Caption}
    \label{fig:multi-agent}
\end{figure*}

==> figures/single_agent.tex <==
\begin{figure*}[h!]
    \centering 
    \begin{subfigure}[b]{.48\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{assets/multi-agent-eval.pdf}  
         \caption{ }
         \label{fig:single-agent:train}
     \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{assets/multi-agent-eval.pdf}  
         \caption{ }
         \label{fig:single-agent:val}
     \end{subfigure}
    \caption{Caption}
    \label{fig:single-agent}
\end{figure*}

==> old_drafts/nuerips/abstract.tex <==
 
\begin{abstract} 
    The training, testing, and deployment, of autonomous vehicles requires accurate, realistic, and efficient simulators. More-over, because of the high variability between different problems presented in different autonomous systems, these simulators need to be easy to use, and easy to modify. Lastly, because many modern algorithms rely on computation graphs and gradient based optimization, efficiently learning from simulation can often require differentiability. To address these problems, we present TorchDriveEnv, an extension the TorchDriveSim package. TorchDriveEnv includes a suite of fully differentiable policy learning benchmarks, which can each be easily modified to test a number of different factors in learned vehicle behaviours including: the effect of varying kinematic models, agent types, and traffic control patterns. Most importantly, unlike many replay based simulation approaches, TorchDriveEnv is fully integrated with Inverted AI service on NPCs initialization and generating realistic driving behaviors for them. This means that simulation remains both realistic, and can be easily modified to increase task difficulty through the addition of additional (data-driven) external agent initializations. 
\end{abstract}
 
% The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.

==> old_drafts/nuerips/baselines.tex <==
\section{Baseline Experiments}


\begin{figure}
    \centering
    % \includegraphics{}
    \caption{This figure should contain RL algorithms with standard hyper-parameters run on the benchmark, we can report information like min/max/mean reward + number of waypoints found + anything else being logged (off-road infractions ext.).}
    \label{fig:enter-label}
\end{figure}


==> old_drafts/nuerips/design.tex <==


\include{tables/table_1}

\section{Design}

\subsection{Simulator}
The simulated world consists of the following elements: {\color{red} this should have a figure illistrating most of these.}
\begin{itemize}
\item Static background, by default including road (derivable surface) and lane markings, represented as a triangle mesh.

\item Control elements, represented by rectangles with internal state. The simulator does not enforce their semantics.

\item A collection of agents grouped into arbitrary types. All agents are visually represented as rigid rectangles.

\item Per agent type kinematic models, defining the agents’ action space and how actions translate into motion.

\item A configurable renderer, displaying the world from a bird’s eye view (birdview), using a customizable color map.
\end{itemize}


Each agent is described by its static attributes (length, width, and others as needed by kinematic models), dynamic state (x, y, orientation, speed), and a flag (present mask) indicating whether a given agent is currently alive. At each time step, the agents perform actions, which in turn determine their next state. The simulator allows the agents to overlap, which is identified as a collision but not prohibited, and the states of different agents do not influence each other except through the agents’ actions. The simulator can operate either in homogeneous mode (all agents are the same type and their states and actions are tensors), or in heterogeneous mode (there are multiple agent types and their states and actions are dictionaries mapping agent types to tensors). To support both modes, most operations are applied as functors, which lift a function acting on a single agent type into a function acting on all agent types. However, this behavior should be transparent to users who do not modify the simulator code.

The base simulator requires actions for all agents and does not modify their presence masks. For convenience, we provide various wrappers modifying the simulator’s behavior, such as by controlling a subset of agents (by replay or pre-defined controllers), removing agents that exit the designated area, monitoring infractions, recording video, and many others. Unless specified otherwise, the wrappers can be combined in different orders to reach desired effects.

\paragraph{Maps and Map Formats}

TorchDriveSim uses Lanelet2 as its map format, but it runs without Lanelet2 on any of the pre-defined maps available as meshes in this repo. However, it won’t be able to detect wrong-way infractions and use certain heuristic behavioral models. To use those features and TorchDriveSim with your own maps, you will need to install Lanelet2 with its Python bindings. You can either use the official distribution or the fork hosted by Inverted AI, which allows for installation without ROS.



\paragraph{Kinematic models}
The primary kinematic model for vehicles in TorchDriveSim is the bicycle model, where the action consists of steering and acceleration. It requires additionally specifying the rear axis offset to control the vehicle turn radius, but it does not use the front axis offset, since that can not be fit by observing the vehicle movement from the outside, effectively assuming the front axis is in the middle of the vehicle. Other kinematic models available are the unconstrained model, where the action is the state delta between subsequent time steps, and the teleporting model, where the action directly specifies the next state. We also provide different variations of those models, and it is straightforward to implement a custom one.

\paragraph{Traffic Controls}


\paragraph{Differentiable rendering}
TorchDriveSim supports two rendering backends, namely Pytorch3D \citep{} and nvdiffrast \citep{}, both producing results that look the same to the human eye. Pytorch3D is the default one and a required dependency since it’s easier to install. Nvdiffrast is supported and can sometimes be substantially faster, but it needs to be installed separately, and it’s subject to more restrictive license conditions. We also provide a dummy rendering backend that returns an empty image, mostly for debugging and benchmarking purposes.



\subsection{Behavior}

The hardest driving scenarios are those that require interactions with other road users. When building simulated environments it is crucial to ensure that the other agents behave realistically, but achieving that is not easy and TorchDriveSim is flexible in terms of how those other agents are controlled. We provide a simple heuristic that achieves minimally sensible driving, noting that in most cases it will be unsatisfactory and require additional extensions. We also facilitate log replay and demonstrate how to use recorded actions from the INTERACTION dataset. However, such replay is not reactive, often resulting in spurious collisions.

For maximum realism and reactivity, we recommend using our (Inverted AI) API for generating realistic behaviors, which is integrated with TorchDriveSim. This is a paid offering that requires an API key, which you can obtain by contacting us. For academics, we may be able to offer free API keys.

Inverted AI API provides a service that controls non-playable characters (NPCs) in driving simulations. The two main functions are INITIALIZE, called at the beginning of the simulation, and DRIVE, called at each time step. Typically, the user runs their simulator locally, controlling the actions of the ego vehicle, and querying the API to obtain the behavior of NPCs. This page describes the high level concepts governing the interaction with the API. Please refer to specific pages for Python SDK, C++ SDK, REST API, Getting started, and Examples.

The core interface is a REST API, that can be called from any programming language. This is a low-level, bare-bones access mode that offers maximum flexibility to deploy in any environment. For convenience, we also provide a Python SDK, freely available on PyPI with minimal dependencies, which provides an abstraction layer on top of the REST API. Recently, we also released C++ SDK and in the future we intend to release similar libraries for other languages.

We follow the continuous space, discrete time approach used in most driving simulators. In the current version, the API only supports a time step of 100 ms, corresponding to 10 frames per second, and expects to run in a synchronous fashion. The latency of API calls varies with physical location of the client server and its network configuration, but generally the API should not be relied upon to provide real-time simulation. For optimal resource utilization, we recommend that you run multiple simulations in parallel, so that one can execute when another is waiting for the API reply. The technology underlying the API is based on ITRA and was optimized to handle simulations of up to 20 seconds (200 time steps) contained within an area of roughly 300 meters in diameter. The API backend has been provisioned to accommodate a large number of agents, where the maximum allowed varies per location.

\subsubsection{INITIALIZE}

Initializes a simulation in a given location, using a combination of user-defined and sampled agents. User-defined agents are placed in a scene first, after which a number of agents may be sampled conditionally.  Conditionally sampled agents can have their agent type specified. Initialize is traffic light state aware. If traffic lights are present in the scene their states should be specified in order to ensure sensible static traffic arrangement sampling..

\subsubsection{DRIVE}

We represent the instantaneous state of each vehicle as four numbers: x and y position, orientation angle, and speed. We do not consider lateral velocity, vehicle lights, or any other information about vehicle state. DRIVE predicts the next state for each vehicle, rather than an action that can be executed in the local simulator and run through its dynamics model. The predicted motion is consistent with the kinematic bicycle model and accelerations are constrained to a reasonable range observed in real world traffic, but there is no guarantee that the corresponding motion could be realized through some action given a particular dynamics model in the local simulator. We recommend teleporting the NPCs to their new positions, since any discrepancies between predicted and realized states for NPCs may negatively affect the quality of subsequent predictions.

Currently the API only supports a general vehicle class and pedestrians, but future releases will add bicycles, and discriminate between vehicle types, such as car, bus truck among others. Vehicles are assumed to be rigid rectangles with a set length and width. The motion of each vehicle is constrained by the kinematic bicycle model, which further requires specifying axle offsets, which is simplified to the distance between the center of the vehicle and its rear axis, referred to as the ``rear axis offset''. While a front axis offset also exists, it is extremely challenging to fit this accurately from observational data, so it is omitted. 

\subsection{Environment}
We proceed to define an environment, which we call TorchDriveEnv. TorchDriveEnv encompasses TorchDriveSim as the core simulator, and bunldes this with API based behavioral models for initialization and reactive motion, both described in \cref{sec:asdf}. It is then augmented with a reward based on infraction metrics and waypoints, and comes with pre-defined training and validation scenarios, as well as the option to use external data and a scenario editor to create hand tailored new scenarios. An overview of its primary components is given in the following.


\paragraph{Scenario Definition}
\begin{table}[h!]
     \begin{center}
     \begin{tabular}{ c  p{10cm}}
     \toprule
      Birdview & Description\\ 
    \cmidrule(r){1-1}\cmidrule(lr){2-2}
     \raisebox{-\totalheight}{\includegraphics[width=40mm, height=40mm]{figures/roundabout.png}}
      & 
      \begin{itemize}[topsep=0pt]
      \item roundabout \ldots
      \end{itemize}\\ 
    \cmidrule(r){1-1}\cmidrule(lr){2-2}
     \raisebox{-\totalheight}{\includegraphics[width=40mm, height=40mm]{figures/traffic_lights.png}}
      & 
      \begin{itemize}[topsep=0pt]
      \item traffic lights \ldots
      \end{itemize}\\ 
    \cmidrule(r){1-1}\cmidrule(lr){2-2}
     \raisebox{-\totalheight}{\includegraphics[width=40mm, height=40mm]{figures/parked_car_yield_stop_sign.png}}
      & 
      \begin{itemize}[topsep=0pt]
      \item a preset parked car in front of the start position of the ego car, and the following waypoints are behind the parked car
      \item yield sign
      \item stop sign \ldots
      \end{itemize}\\ 
    \cmidrule(r){1-1}\cmidrule(lr){2-2}
     \raisebox{-\totalheight}{\includegraphics[width=40mm, height=40mm]{figures/3_ways.png}}
      & 
      \begin{itemize}[topsep=0pt]
      \item three-way intersection
      \item merge with a preset car into a lane with preset traffic \ldots
      \end{itemize}\\ 
    \cmidrule(r){1-1}\cmidrule(lr){2-2}
     \raisebox{-\totalheight}{\includegraphics[width=40mm, height=40mm]{figures/chicken.png}}
      & 
      \begin{itemize}[topsep=0pt]
      \item a car is overtaking another car in the opposite direction, and thus both lanes of the road are occupied\ldots
      \end{itemize}
      \\ \bottomrule
      \end{tabular}
      \caption{Validation Scenario Cases}
      \label{tbl:myLboro}
      \end{center}
\end{table}

% NOTE: this should contain a description of the scenarios that come bundled with it. i.e. 1000 training scenarios, and 10 validation scenarios
With maps and behavioral models available, the final hurdle is to define a suite of driving scenarios that can be used for testing and evaluation. TorchDriveSim provides helpers for initializing the simulation state, including by calling Inverted AI API, instantiating from a log (when available), and using some simple heuristics. It also provides functions for identifying driving infractions, specifically collisions, going off-road, and driving the wrong way. However, it does not specify goals or rewards, leaving that to the user. Over time, we are planning to release various scenario suites that can serve as benchmarks. 

\subsubsection{Initialization}

\subsubsection{Stepping}

\subsubsection{Action Space}
Continuous action space: steering $b$, acceleration $c$, kinetic model: Bicycle model
\begin{align*}
b \in (-0.3, 0.3) \\
c \in (-1.0, 1.0) 
\end{align*}


\subsubsection{Observation Space}
A $3 \times 3 \times 64 \times 64$ matrix indicating 3 frames of the bird view images


\subsubsection{Reward}

TorchDriveEnv is a partially observable Markov decision process in the sense that the intents and actions of non-ego agents are not observable.  This POMDP is, in the standard approimation way, reduced to an MDP in which the policy is conditioned on a deterministically extracted belief state from a stack of recent observations.  In this case, the ego-agent is conditioned on a ``state'' consisting of concatenated bird view images showing a map and the current (at each time) 

\begin{align*}
s_t &\in \mathcal{S}\\
a_t &\in \mathbb{R}^2\\
w_t &\in \mathbb{R}^2\\
x_t &\in \mathbb{R}^2\\
p(s_{t+1}|s_t,a_t) 
\end{align*}
  Here $s_t$ is a stack of 3 frames and ...





\[\text{Reward} = \text{Distance} + \text{Reach Target}\]

\begin{align*}
    r_t =  &\mathbbm{1}\left(d(s_t, s_{t+1}) > \epsilon_0\right) \\ 
&+ \lambda_0 \mathbbm{1}(d(s_{t+1}, w_i(s_{1:t})) < \epsilon_1) \\ 
&+ \lambda_1\mathbbm{1}(f_{\text{offroad}}(s_{t+1}) )\\ 
&+ \lambda_2\mathbbm{1} (f_{\text{wrong\_way}}(s_{t+1}) ) \\
&+ \lambda_3\mathbbm{1}(f_{\text{traffic\_light\_violation}}(s_{t+1})) \\
&+ \lambda_4\mathbbm{1} (f_{\text{collision}}(s_{t+1}) )\\
&\rightarrow + \lambda_5(1-\cos(\psi_t - \psi_{t+1}))
\end{align*}
\begin{align*}
T &= 200 \\
\epsilon_0 &= 0.5 \\
\epsilon_1 &= 3 \\ 
\lambda_0 &= 30  \rightarrow 10\\
\lambda_1 &= -10 \rightarrow 0\\
\lambda_2 &= -10 \rightarrow 0\\
\lambda_3 &= -10 \rightarrow 0\\
\lambda_4 &= -10 \rightarrow 0\\
\lambda_5 &= -0.05
% TODO: 
\end{align*}




==> old_drafts/nuerips/discussion.tex <==
\section{Discussion}

==> old_drafts/nuerips/introduction.tex <==
\section{Introduction}

In the last decade, autonomous vehicles have gone from academic obscurity to one of the biggest sector in the technology industry~\cite{}. This is in no small part due to the improvements to autonomous vehicle simulation~\cite{}, and the rapid evolution of deep learning~\cite{}. In almost all modern systems for training or testing of autonomous vehicles, simulation plays a crucial role. This is because both training and testing on real world hardware is not only expensive and time-consuming, but represents a legitimate danger to public safety~\cite{}. Therefore companies and research groups like~\cite{}, have placed progressively more effort into producing simulators which are more realistic and efficient to use. In many cases, these simulators have allowed both academic researchers as well as industry professionals to solve a number of open problems in autonomous control~\cite{}, and even computer vision~\cite{}. However even many modern simulators ignore the current technical requirements for both the training and testing of complex controllers, which may need to satisfy a range of different engineering requirements~\cite{}. More specifically, existing autonomous vehicle simulators often lack realism and are not easy to modify as requirements for controller training and testing change. Additionally, many of these simulators have ignored advances in computation graphs and deep-learning that make learning better policies easier~\cite{}. 

In order to address these issues, we present TorchDriveEnv. Based on TorchDriveSim, a lightweight 2D driving simulator, built entirely in PyTorch, TorchDriveEnv is primarily intended as a training environment for developing autonomous driving algorithms. Unlike many existing simulation environments, TorchDriveEnv provides realistic external agents, and is fully differentiable. More specifically, TorchdriveEnv provides fully differentiable execution producing, which produces a single computation graph which includes state transition information (based upon kinematic models) and observation information (defined by a differentiable rendering). Notably, the kinematic models which define the underlying transitions of TorchDriveEnv, can be easily modified or customized (unconstrained, unicycle, bicycle, etc.), as can the differentiable, rendered observations. Whats more, metrics of interest like collisions, off-road, and wrong way infractions are also fully differentiable. For ease of use in model training and evaluation, TorchDriveEnv also provides first class support for batch processing, and is defined by a modular collection of wrappers which can change simulator behaviour, similar to~\cite{}. In fact, TorchDriveEnv follows current standard in reinforcement learning environments in terms of the step and reset functions, making integration with RL benchmarking libraries like~\cite{} simple. 

TorchdriveEnv also also allows for more diverse traffic environments through the use of heterogeneous agent types (vehicles, pedestrians, cyclists, etc.), each with its own kinematic model. Direct control over traffic control information like traffic lights is also included in order to further improve realism. Lastly, and most importantly, TorchdriveEnv is integrated with the Inverted AI API, and can dynamically initialize agent state information and provide realistic driving behaviours.  This means that given a specific map~\cite{}, the user can easily vary not just the number of external agents included in simulation, but can also rely on TorchdriveEnv to place them in a data-driven fashion. These external agents can then be controlled using data-driven behavioural models~\cite{} to create realistic, stochastically generated driving scenarios. This user controlled scenario modification, thus allows for more or less complex training and testing of multi-agent autonomous vehicle controllers. In the following sections, we will illustrate how this simulator functions, how it can be used or modified, and finally some of the advantages it offers over comparable simulators. We conclude with a discussion of the policy learning benchmarks included in TorchDriveEnv, and show how easy training and testing can be. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.19\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.19\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.19\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.19\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.19\textwidth]{placeholder-1024x1024.png}
    \caption{\color{red} This set of examples should show for a static set of initial conditions the different types of behaviours we can sample.  -- INITIALIZE visualization}
    \label{fig:div-ex}
\end{figure}

\begin{itemize}[leftmargin=0.65cm] \itemsep0em   
     % \item Fully differentiable execution producing a single computation graph, including state transition (kinematic models) and observation (differentiable rendering) models.
    % \item First class support for batch processing, down to the lowest level.
    % \item Support for heterogeneous agent types (vehicles, pedestrians, cyclists, etc.), each with its own kinematic model.
    % \item Extensible and customizable implementation of kinematic models (unconstrained, unicycle, bicycle, etc.), rendering modes, and rendering backends.
    % \item Support for extensible traffic control types, including traffic lights.
    % \item Differentiable implementations of various infraction metrics (collisions, off-road, wrong way).
    % \item Modular collection of wrappers modifying the simulator’s behavior.
    \item \color{red} Ability to ingest any map in Lanelet2 format out of the box.
    % \item Integration with IAI API for initializing agent states and providing realistic behaviors.
\end{itemize}



% Its main features are:

% simulation is has been an important part of vehicile lerarning for a while
% now its crucial to testing and training
% as problems get harder we need to make better av controllers
% to do this we need better simulators that fit the current training landscape
% these controllers need to fit the following criteria
% torchdriveenv does this and more

% we the included benchmarks test the following scenarios 

% you can make them harder or easiers based on whatever

% all tech is based from the inverted ai simulator

% iai sim is the best becuase we built it with data 

% below we illistrate how to use these benchmarks for testing and traing

% we also give basic examples of why you should use this over others (like increased initialization waypoint placement whatever).

% we conclude by comparing existing systems an algorithms on our benchmarks to show how perf can vary 


% Simulation is a key component for achieving Level 5 full driving automation. This is because testing in the real world is both slow and costly and more importantly dangerous for public safety. 


% TorchDriveSim is a lightweight 2D driving simulator, built entirely in PyTorch, primarily intended as a training environment for developing autonomous driving algorithms. Its main features are:

% \begin{itemize}
%     \item Fully differentiable execution producing a single computation graph, including state transition (kinematic models) and observation (differentiable rendering) models.
%     \item First class support for batch processing, down to the lowest level.
%     \item Support for heterogeneous agent types (vehicles, pedestrians, cyclists, etc.), each with its own kinematic model.
%     \item Extensible and customizable implementation of kinematic models (unconstrained, unicycle, bicycle, etc.), rendering modes, and rendering backends.
%     \item Support for extensible traffic control types, including traffic lights.
%     \item Differentiable implementations of various infraction metrics (collisions, off-road, wrong way).
%     \item Modular collection of wrappers modifying the simulator’s behavior.
%     \item Ability to ingest any map in Lanelet2 format out of the box.
%     \item Integration with IAI API for initializing agent states and providing realistic behaviors.
% \end{itemize}














==> old_drafts/nuerips/related.tex <==

\section{Related Work}
Recent years have seen a major surge in autonomous vehicle simulation, and this increased interest has led to progressively more realistic simulation environments~\cite{dosovitskiy2017carla,muller2018sim4cv,cai2020summit}. In many cases these simulators were originally constructed to reduce the so called simulation to reality gap~\cite{tobin2017domain,osinski2020simulation,bewley2019learning,muller2018driving}, which is charactorized by how well controllers learned in simulation function in a real world setting. Eventually, many of these simulators have evolved, or been used to create machine learning and control benchmarks which can test a number of different policy learning problems~\cite{dosovitskiy2017carla,zhan2019interaction,codevilla2019exploring}. Many of these simulators and benchmarks test performance in multi agent environments where external (non-ego) agents are executed using either rule based setups~\cite{treiber2000congested,likmeta2020combining,xiao2021rule} or by replaying historical data~\cite{vinitsky2022nocturne,li2022metadrive, caesar2021nuplan}. Many of these multi-agent autonomous vehicle benchmarks have been tailored for image based deep learning systems, and can test a variety of algorithm classes~~\cite{muhammad2020deep,zuo2017continuous}. In some cases, these benchmarks include historical data which can be used for learning via behavioural cloning~\cite{bansal2018chauffeurnet,pomerleau1988alvinn,bojarski2016end,rhinehart2019precog,codevilla2018end,chen2020learning}. In other cases only local (non-expert) information is included like reward or infraction info, and algorithms tested usually boil down to some form of reinforcement learning~\cite{kendall2019learning,isele2018navigating,wang2018reinforcement,lu2023imitation} or  decision transformers~\cite{fu2022decision,dong2022development}. Such benchmarks can also often intermingle feedback, and many researchers test algorithms like  inverse reinforcement learning~\cite{igl2022symphony,bronstein2022hierarchical,lee2020mixgail,couto2021generative} in these simulated environments as well. Other approaches more related to control have also been investigated in these benchmarks and simulators, specifically trajectory prediction~\cite{chai2019multipath,tang2019multiple, liang2020learning, ngiam2021scene, gu2021densetnt, nayakanti2023wayformer} and learning safe autonomous vehicle controllers~\cite{vitelli2022safetynet}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.235\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.235\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.235\textwidth]{placeholder-1024x1024.png}
    \includegraphics[width=0.235\textwidth]{placeholder-1024x1024.png}
    \caption{\color{red} This should be a single scene where we plot what the different external agent trajectories look like to illustrate why its diverse. -- ITRA visualization}
    \label{fig:enter-label}
\end{figure}

%%%%%%%%%%%%%%%%%%%
% sim 2 real  ---
%%%%%%%%%%%%%%%%%%%
% Domain Randomization for Transferring Deep Neural Networks from Simulation to the Real World tobin2017domain
% Simulation-based reinforcement learning for real-world autonomous driving osinski2020simulation
% Learning to drive from simulation without real world labels bewley2019learning
% Driving policy transfer via modularity and abstraction muller2018driving

%%%%%%%%%%%%%%%%%%%
% benchmarks ---
%%%%%%%%%%%%%%%%%%%
% interaction dataset zhan2019interaction
% CARLA / CoRL 2017 
% Exploring the limitations of behavior cloning for autonomous driving codevilla2019exploring

%%%%%%%%%%%%%%%%%%%
% realistic physics / photo-realism ---
%%%%%%%%%%%%%%%%%%%
% CARLA \cite{dosovitskiy2017carla} 
% Sim4cv: A photo-realistic simulator for computer vision applications. \cite{muller2018sim4cv}
% Summit: A simulator for urban driving in massive mixed traffic \cite{cai2020summit}

%%%%%%%%%%%%%%%%%%%
% importance of deeplearning in AV --
%%%%%%%%%%%%%%%%%%%
% Deep learning for safe autonomous driving: Current challenges and future directions muhammad2020deep
% Continuous reinforcement learning from human demonstrations with integrated experience replay for autonomous driving

%%%%%%%%%%%%%%%%%%%
% autonomous vehicle learning data-sets behavior
%%%%%%%%%%%%%%%%%%%
% Large scale interactive motion forecasting for autonomous driving : The waymo open motion dataset. 
% interaction dataset zhan2019interaction

%%%%%%%%%%%%%%%%%%%
% replay based simulation ---
%%%%%%%%%%%%%%%%%%%
% Nocturne: a scalable driving benchmark for bringing multi-agent learning one step closer to the real world. vinitsky2022nocturne
% Metadrive: Composing diverse driving scenarios for generalizable reinforcement learning. li2022metadrive
% A closed-loop ml-based planning benchmark for autonomous vehicles caesar2021nuplan

%%%%%%%%%%%%%%%%%%%
% rule based simulation --
%%%%%%%%%%%%%%%%%%%
% Congested traffic states in empirical observations and microscopic simulations.  treiber2000congested
% Combining reinforcement learning with rule-based controllers for transparent and general decision-making in autonomous driving likmeta2020combining
% Rule-based Optimal Control for Autonomous Driving xiao2021rule

%%%%%%%%%%%%%%%%%%%
% behavioral cloning ---
%%%%%%%%%%%%%%%%%%%
% Learning to drive by imitating the best and synthesizing the worst. bansal2018chauffeurnet
% An autonomous land vehicle in a neural network. pomerleau1988alvinn
% End to end learning for self-driving cars bojarski2016end
% PRECOG: prediction conditioned on goals in visual multi-agent settings rhinehart2019precog
% End-to end driving via conditional imitation learning. codevilla2018end
% Learning by cheating. chen2020learning

%%%%%%%%%%%%%%%%%%%
% trajectory prediction -- predict trajectories of other vehicles
%%%%%%%%%%%%%%%%%%% 
% Multipath: Multiple probabilistic anchor trajectory hypotheses for behavior prediction chai2019multipath
% Multiple futures prediction tang2019multiple
% Learning lane graph representations for motion forecasting liang2020learning
% Scene transformer: A unified architecture for predicting multiple agent trajectories. ngiam2021scene
% End-to-end trajectory prediction from dense goal sets.
% Wayformer: Motion forecasting via simple & efficient attention networks  nayakanti2023wayformer

%%%%%%%%%%%%%%%%%%%
% inverse reinforcement learning ---
%%%%%%%%%%%%%%%%%%%
% Symphony: Learning realistic and diverse agents for autonomous driving simulation. igl2022symphony
% Hierarchical model-based imitation learning for planning in autonomous driving bronstein2022hierarchical
% GAIL  lee2020mixgail, couto2021generative

%%%%%%%%%%%%%%%%%%%
% reinforcement learning ---
%%%%%%%%%%%%%%%%%%%
% Learning to drive in a day kendall2019learning
% Navigating occluded intersections with autonomous vehicles using deep reinforcement learning. isele2018navigating
% A reinforcement learning based approach for automated lane change maneuvers.  wang2018reinforcement
% Imitation is not enough: Robustifying imitation with reinforcement learning for challenging driving scenarios. lu2023imitation

%%%%%%%%%%%%%%%%%%%
% Safe-AV
%%%%%%%%%%%%%%%%%%%%
% Safetynet: Safe planning for real-world self-driving vehicles using machine-learned policies. vitelli2022safetynet


==> old_drafts/nuerips/tables/table_1.tex <==
\begin{table*}[t]
\footnotesize
\setlength{\tabcolsep}{1mm}
\centering
% \def\arraystretch{1.2}
\begin{tabular}{lc|c|c|c|c|c|c}
\specialrule{.2em}{.1em}{.1em}
& Multi-agent & Accel. & Sensor Sim & Expert Data & Sim-agents & Real Data & Routes/Goals \\
\hline
TORCS~\cite{wymann2000torcs} & 
  & 
 & % Graphics & 
\cmark & 
 & 
\cmark &
 & 
 - \\
GTA V~\cite{martinez2017beyond} & 
 & 
 & % Graphics & 
\cmark &
 & 
 &
 & 
 - \\
CARLA~\cite{dosovitskiy2017carla} & 
 & 
 & % Graphics & 
\cmark & 
 & 
\cmark & 
 & 
Waypoints \\
Highway-env~\cite{highway-env} & 
 & 
 & 
 &
 & 
 &
 & 
- \\
Sim4CV~\cite{muller2018sim4cv} & 
 & 
 & % Graphics & 
\cmark & 
 & 
 &
 &
Directions\\
SUMMIT~\cite{cai2020summit} & 
\cmark ($\geqslant400$) & 
 & % Graphics & 
\cmark & 
 & 
\cmark &
\cmark &
- \\
MACAD~\cite{palanisamy2020multi} & 
\cmark & 
 & % Graphics & 
\cmark & 
 & 
\cmark &
 & 
Goal point\\
DeepDrive-Zero~\cite{craig_quiter_2020_3871907} &
\cmark & 
 & 
 &
 & 
\cmark &
 & 
- \\
SMARTS~\cite{zhou2020smarts} & 
\cmark & 
 & 
 & 
 & 
 & 
 & 
Waypoints \\
MADRaS~\cite{santara2021madras} & 
\cmark ($\geqslant10$) & 
 & % Graphics &
\cmark & 
 & 
\cmark &
 & 
Goal point\\
DriverGym~\cite{kothari2021drivergym}& 
 & 
 & 
 & 
\cmark &
\cmark & 
\cmark &
- \\
VISTA~\cite{amini2022vista} &
\cmark & 
 & % Graphics & 
\cmark &
\cmark & 
 &
 & 
- 
\\
nuPlan~\cite{caesar2021nuplan} &
 & 
& 
\cmark & 
\cmark & 
\cmark & 
\cmark & 
Waypoints
\\
Nocturne~\cite{vinitsky2022nocturne}& 
\cmark ($\geqslant50$) & 
 &
 &
\cmark & 
\cmark & 
\cmark & 
Goal point \\
MetaDrive~\cite{li2022metadrive} &
\cmark &
 &
\cmark &
\cmark &
\cmark &
\cmark &
- 
\\
Intersim~\cite{sun2022intersim} & 
\cmark & 
 & 
 & 
\cmark & 
\cmark &
\cmark & 
Goal point \\
TorchDriveSim~\cite{itra2021} & 
\cmark & 
\cmark & 
 & 
 & 
\cmark &
 & 
- \\
tbsim~\cite{xu2022bits} & 
\cmark & 
 & 
 & 
\cmark & 
\cmark &
\cmark & 
Goal point \\
\waymax (ours) & 
\cmark ($\geqslant128$) & 
\cmark & 
 &
\cmark & 
\cmark & 
\cmark &
Waypoints
\\
\specialrule{.1em}{.05em}{.05em}

\end{tabular}
\caption{\label{table:related}A comparison of related driving simulators (chronological order).
\emph{Multi-agent.}: Simulating multiple agents. Supported number of agents are in the parentheses (if available). \emph{Accel.}: In-graph compilation for hardware (GPU/TPU) acceleration.
\emph{Sensor Sim}: Sensors (e.g. camera, lidar \& radar) input simulation.
\emph{Expert Data}: Human demonstrations or rollout trajectories collected with an expert policy.
\emph{Sim-agents}: agent models for simulated objects (e.g. other vehicles).
\emph{Real data}: Real world driving data.
\emph{Routes/Goals}: "$-$" means no routes or goals are provided; "Waypoints" means positions sampled from a trajectory; "Directions" means discrete driving directions including left, straight, and right; "Goal point" means the goal position.}
\label{table:simulators}
\color{red} Add differentiability as a column
\end{table*}
